Construction of power flow feasibility sets

We develop a new approach for construction of convex analytically simple regions where the AC power flow equations are guaranteed to have a feasible solutions. Construction of these regions is based on efficient semidefinite programming techniques accelerated via sparsity exploiting algorithms. Resulting regions have a simple geometric shape in the space of power injections (polytope or ellipsoid) and can be efficiently used for assessment of system security in the presence of uncertainty. Efficiency and tightness of the approach is validated on a number of test networks.

==> TPWRS - Feasibility 2015/Definitions.tex <==
%!TEX root=ConvexEnergyFunction.tex

\newcommand{\Sen}[4]{\mathrm{S}_{#2,#1}\br{{#4}}}
\newcommand{\Dcal}{\hat{\cal D}}

%Names
\newcommand{\HJB}{{ HJB}}
\newcommand{\DGs}{{ DGs}}
\newcommand{\DG}{{ DG}}
\newcommand{\LDGs}{{ LDGs}}
\newcommand{\LDG}{{ LDG}}
\newcommand{\Pname}{passive dynamics}
\newcommand{\Ppol}{passive policy}
\newcommand{\LMDP}{{ LMDP}}
\newcommand{\LMDPs}{{ LMDPs}}
\newcommand{\MDPs}{{ MDPs}}
\newcommand{\MDP}{{ MDP}}
\newcommand{\MGs}{{ MGs}}
\newcommand{\MG}{{ MG}}
\newcommand{\LMGs}{{ LMGs}}
\newcommand{\LMG}{{ LMG}}
\newcommand{\LD}{{ LD}}
\newcommand{\LDs}{{ LDs}}
\newcommand{\Pol}{Pol}
\newcommand{\Dyn}{Dyn}
\newcommand{\OptPol}{OP}
\newcommand{\BE}{{ BE}}
\newcommand{\BEs}{{ BEs}}
\newcommand{\Cost}{Co}
\newcommand{\FH}{{\rm FH}}
\newcommand{\FE}{{\rm FE}}
\newcommand{\IH}{{\rm IH}}
\newcommand{\PIC}{{\bf PIC}}
\newcommand{\LGs}{{\bf $\alpha$-RLCs}}
\newcommand{\LG}{{\bf $\alpha$-RLC}}
\newcommand{\Ren}{Renyi~}
\newcommand{\Pipasname}{Null Policy}
\newcommand{\CCDa}[1]{~\mathrm{CCS}_1\left({#1}\right)}
\newcommand{\CCDb}[1]{~\mathrm{CCS}_2\left({#1}\right)}
\newcommand{\Sop}{\mathrm{SUBOPT}}
\newcommand{\CON}{\rm{CON}}
\newcommand{\NCON}{\rm{NCON}}
\newcommand{\Aut}{\rm{AUT}}
\newcommand{\OPT}{\rm{OPT}}
\newcommand{\D}{\mathcal{D}}



%% General  Math Notation   %%

%Singular Values/Eigenvalues
\newcommand{\la}[1]{\lambda\left({#1}\right)}
\newcommand{\lai}[2]{\lambda_{#2}\left({#1}\right)}
\newcommand{\lam}[1]{\lambda_{\min}\left({#1}\right)}
\newcommand{\lama}[1]{\lambda_{\max}\left({#1}\right)}
\newcommand{\sva}[1]{\sigma\left({#1}\right)}
\newcommand{\svai}[2]{\sigma_{#2}\left({#1}\right)}
\newcommand{\svam}[1]{\sigma_{\min}\left({#1}\right)}
\newcommand{\svama}[1]{\sigma_{\max}\left({#1}\right)}

\newcommand{\ind}[1]{\mathsf{I}\left[{#1}\right]}
\newcommand{\brs}[1]{\left[{#1}\right]}

%Optimality
\newcommand{\opt}[1]{{#1}^\ast}
\newcommand{\optt}[1]{{{#1}_c}^\ast}

%Miscellaneous Functions
\DeclareMathOperator*{\subsetm}{\subset^m}
\DeclareMathOperator{\sign}{\mathrm{sign}}
\newcommand{\sgn}[1]{\mathrm{sgn}\br{{#1}}}
\DeclareMathOperator{\LogSumExp}{\Psi}
\DeclareMathOperator*{\mini}{\text{Minimize}}
\DeclareMathOperator*{\maxi}{\text{Maximize}}
\DeclareMathOperator*{\argmin}{{ \sf{argmin}}}
\DeclareMathOperator*{\argmax}{{\sf{argmax}}}
\DeclareMathOperator{\ntimes}{\otimes}
\newcommand{\logp}[2]{\LogSumExp_{#1}\left[{#2}\right]}
\newcommand{\logpa}[3]{\LogSumExp^{#3}_{#1}\left[{#2}\right]}
\newcommand{\fpert}[3]{{\bar{#1}}\br{#3}}
\newcommand{\fpertr}[3]{{\tilde{#1}}_{#2}\br{{#3}}}
\newcommand{\logpaw}[4]{{#4}_{{#3}}\br{{#2}}}
\newcommand{\expb}[1]{\exp\left({#1}\right)}
\newcommand{\logb}[1]{\log\left({#1}\right)}
\newcommand{\norm}[1]{\left\lVert {#1} \right\rVert}
\newcommand{\Reg}[1]{R\left({#1}\right)}
\newcommand{\ord}[2]{{#1}_{\left[{#2}\right]}}
\newcommand{\abs}[1]{\left|  {#1}  \right|}
\newcommand{\powb}[2]{{\left({#1}\right)}^{#2}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\One}{\mathbf{1}}
\newcommand{\tran}[1]{{#1}^T}
\newcommand{\Set}[1]{\left\{{#1}\right\}}
\newcommand{\inner}[2]{\left\langle {#1},{#2} \right\rangle}
\newcommand{\Rad}[1]{\mathrm{R}\br{#1}}
\newcommand{\Scal}{\mathcal{S}}


%Derivatives
\DeclareMathOperator{\der}{\mathrm{d}}
\DeclareMathOperator{\pder}{\partial}
\newcommand{\diff}[1]{\der{#1}}
\newcommand{\pdiff}[1]{\pder{#1}}
\newcommand{\DiffGen}[1]{\DiffG\left[{#1}\right]}
\newcommand{\Diff}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\DDiff}[2]{\frac{\partial^2 {#1}}{\partial {#2} \tran{\partial {#2}} }}



%%Spaces
\newcommand{\Rnn}{\R^{n \times n}}
\newcommand{\Snn}{\mathcal{S}^{n \times n}}
\newcommand{\Pspace}[1]{\mathcal{P}\left[{#1}\right]}
\newcommand{\Poss}[1]{{{#1}}^{\R^+}}
\newcommand{\Fspace}[1]{\mathcal{F}\left[{#1}\right]}
\newcommand{\meso}{\mu_0}
\newcommand{\mes}{\mu}
\newcommand{\mesp}{\nu}



%Probability stuff
\DeclareMathOperator*{\Es}{\mathrm{E}}
\DeclareMathOperator*{\Covs}{\mathrm{Cov}}
\DeclareMathOperator*{\Vars}{\mathrm{Var}}
\DeclareMathOperator{\vari}{\mathbb{\sigma}}
\DeclareMathOperator{\KLs}{\mathrm{KL}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\reg}{\mu}
\newcommand{\Vari}[1]{\mathrm{Var}\left({#1}\right)}
\newcommand{\Covb}[1]{\mathrm{Cov}\left({#1}\right)}
\newcommand{\Var}[2]{\Vars_{{#1}}\left({#2}\right)}
\newcommand{\Gauss}[2]{\N\left({#1},{#2}\right)}
\newcommand{\ExP}[2]{\Es_{{#1}}\left [{#2}\right ]}
\newcommand{\Ent}[1]{H\left [{#1}\right ]}
\newcommand{\Prob}[2]{\Pr_{{#1}}\left [{#2}\right ]}
\DeclareMathOperator{\supo}{\mathrm{supp}}
\newcommand{\KL}[2]{\KLs\left({#1 }\parallel {#2}\right)}
\newcommand{\Div}[2]{\mathrm{Div}\left({#1 }\parallel {#2}\right)}
\newcommand{\Dalpha}[2]{\Dal\left({#1 }\parallel {#2}\right)}
\newcommand{\UN}{\tilde{\mathcal{N}}}
\newcommand{\UNQ}{\UN_Q}
\newcommand{\supp}[1]{\supo\left [{#1}\right ]}
\newcommand{\Prjo}[1]{\mathrm{Proj}_0\left({#1}\right)}
\newcommand{\Proj}[2]{\mathrm{Proj}_{{#1}}\left({#2}\right)}
\newcommand{\Cyc}[2]{{#1}_{\langle {#2} \rangle}}
\newcommand{\Cycv}[1]{\mathrm{Cyc}_{\langle {#1} \rangle}}
\DeclareMathOperator{\Drm}{\mathbb{D}}
\DeclareMathOperator{\Dal}{\mathbb{D}_\alpha}
\DeclareMathOperator{\ovec}{\mathbf{\omega}}
\newcommand{\Darg}[3]{\Drm_{#1}\left({#2} \parallel {#3}\right)}
\DeclareMathOperator{\DiffG}{\mathcal{L}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Gb}{\mathbf{G}}

\newcommand{\ic}{\mathbf{j}}


%Matrix stuff

\newcommand{\detb}[1]{\det\left({#1}\right)}
\newcommand{\tranb}[1]{{\left({#1}\right)}^T}
\newcommand{\br}[1]{\left({#1}\right)}
\newcommand{\sqb}[1]{\left[{#1}\right]}
\newcommand{\inv}[1]{{\left(#1\right)}^{-1}}
\newcommand{\inve}[1]{{#1}^{-1}}
\newcommand{\invet}[1]{{#1}^{-T}}
\newcommand{\vecb}[1]{\mathrm{vec}\left({#1}\right)}
\newcommand{\diag}{\mathrm{di}}
\newcommand{\diagb}[1]{\mathrm{di}\left({#1}\right)}
\newcommand{\di}[1]{\mathrm{di}\left({#1}\right)}
\newcommand{\tr}[1]{\mathrm{tr}\left( {#1} \right)}
\newcommand{\stt}{\left[\begin{smallmatrix} \s_t\\ \s_{t+1} \\ 1\end{smallmatrix}\right]}

%% General Controls Notation %%

%Risk
\newcommand{\risk}{\alpha}


%Dimensions
\newcommand{\nc}{n_u}
\newcommand{\ns}{n_s}
\DeclareMathOperator{\Np}{N_+}
\DeclareMathOperator{\Nn}{N_-}
\newcommand{\nn}{p}
\newcommand{\nm}{\mathrm{m}}
\newcommand{\nh}{\mathrm{k}}


%Costs
\newcommand{\costu}{R}
\newcommand{\costn}{\tilde{\ell}}
\newcommand{\costf}{\costt_f}
\newcommand{\costtraj}{\mathcal{L}}
\newcommand{\costr}{\costt_r}
\newcommand{\costw}[2]{\costt\left({#1};{#2}\right)}
\newcommand{\costx}{Q}
\newcommand{\costt}{\ell}
\newcommand{\cost}{\costt_t}
\newcommand{\costJ}{\mathcal{J}}
\newcommand{\costfin}{\costt_f}
\newcommand{\Qcost}{\mathcal{Q}_t}
\newcommand{\costU}{\mathcal{R}}
\newcommand{\costq}{\mathcal{Q}}
\newcommand{\costfq}{q}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\Lm}{\mathcal{L}}
\newcommand{\Lop}{\tilde{L}}
\newcommand{\R}{\mathbb{R}}

%%States, Controls, Trajectories, Noise
\DeclareMathOperator{\co}{\bar{c}}
\newcommand{\s}{x}
\newcommand{\snew}{\s^\prime}
\DeclareMathOperator{\snewy}{\mathbf{y}}
\newcommand{\sv}{\mathbf{s}}
\DeclareMathOperator{\y}{\mathbf{y}}
\DeclareMathOperator{\Traj}{\mathbf{X}}
\newcommand{\noisetraj}{\pmb{\epsilon}}
\newcommand{\noiseutraj}{{\bf \noiseu}}
\newcommand{\trajpr}{\traj^\prime}
\newcommand{\trajp}[1]{\traj_{+}^{({#1})}}
\newcommand{\trajn}[1]{\traj_{-}^{({#1})}}
\newcommand{\traj}{\mathbf{x}}
\newcommand{\uc}{u_c}
\newcommand{\ug}{\mathit{u}}
\newcommand{\ugb}{\mathbf{u}}
\newcommand{\ucb}{\ugb_\mathrm{c}}
\newcommand{\usc}{\ug_{\mathrm{net}}}
\newcommand{\uca}{u}
\newcommand{\uopp}{\ug_\mathrm{a}}
\newcommand{\uoppb}{\ugb_\mathrm{a}}
\newcommand{\uoth}{\tilde{u}}
\newcommand{\uopt}{\uc^\ast}
\newcommand{\Uspace}{\mathcal{U}}
\newcommand{\Uspaceopp}{\mathcal{U}_{\mathrm{a}}}
\newcommand{\Xspace}{\mathcal{X}}%
\newcommand{\yg}{\mathbf{y}}
\newcommand{\ytraj}{\mathbf{y}}
\newcommand{\yb}{\bar{y}}
\newcommand{\noiseu}{\omega}
\newcommand{\noise}{\omega}
\newcommand{\noisew}{\epsilon}



%Horizon
\DeclareMathOperator{\T}{\mathcal{T}}
\DeclareMathOperator{\Tfin}{N_f}
\DeclareMathOperator{\Tex}{N_e}
\DeclareMathOperator{\Th}{N}
\newcommand{\Nh}{N}



%Policies
\newcommand{\Po}{\Pi}
\newcommand{\Pipas}{\Pi^{0}}
\newcommand{\ppr}{P_\mathrm{prior}}
\newcommand{\Ut}[2]{\pic\left({#1}|{#2}\right)}
\newcommand{\Pas}[2]{\Pipas\left({#1}|{#2}\right)}
\newcommand{\PolOpt}[1]{\Po^*\left({#1}\right)}
\DeclareMathOperator{\pic}{\Po_c}
\DeclareMathOperator{\picb}{\mathbf{\Po_c}}
\DeclareMathOperator{\pig}{\Po}
\DeclareMathOperator{\pigb}{\Po}
\DeclareMathOperator{\piopp}{\Po_\mathrm{a}}
\DeclareMathOperator{\pioppb}{\mathbf{\Po}_\mathrm{a}}
\DeclareMathOperator{\piopts}{{\pic}^\ast}
\DeclareMathOperator{\pibopts}{{\picb}^\ast}
\DeclareMathOperator{\pigopts}{{\pig}^\ast}
\DeclareMathOperator{\pigbopts}{{\pigb}^\ast}
\DeclareMathOperator{\pioppopts}{{\piopp}^\ast}
\DeclareMathOperator{\pioppbopts}{{\pioppb}^\ast}
\newcommand{\pigs}[2]{\pig_{#2}\left({#1}\right)}
\newcommand{\piopt}[2]{\piopts\left({#1};{#2}\right)}
\newcommand{\pibopt}[2]{\pibopts\left({#1};{#2}\right)}
\newcommand{\pigopt}[2]{\pig^\ast_{#2}\left({#1}\right)}
\newcommand{\pigbopt}[2]{\pig^{\ast}_{{#2}}\left({#1}\right)}
\newcommand{\pioppopt}[2]{\pioppopts_{{#2}}\left({#1}\right)}
\newcommand{\pioppbopt}[2]{\pioppbopts_{{#2}}\left({#1}\right)}
\newcommand{\piop}[1]{\piopts\left({#1}\right)}
\newcommand{\pigop}[1]{\pigopts\left({#1}\right)}
\newcommand{\pioppop}[1]{\pigopts_\mathrm{a}\left({#1}\right)}
\newcommand{\Polw}[3]{\Po^{#3}\left({#1}|{#2}\right)}
\newcommand{\Polws}[1]{\Po^{#1}}
\newcommand{\PolwT}[2]{\Po^{#2}\left({#1}\right)}
\newcommand{\PolPasT}[1]{\Pipas\left({#1}\right)}
\newcommand{\PolPas}[2]{\Pipas\left({#1}|{#2}\right)}
\newcommand{\PolDet}[2]{\Pi_{{#2}}\left({#1}\right)}


%Value Functions
\newcommand{\valt}[2]{\mathit{v}_{#2}\left({#1}\right)}
\newcommand{\valtw}[3]{\mathit{v}^{{#3}}_{{#2}}\left({#1}\right)}
\newcommand{\valts}[1]{\mathit{v}_{#1}}
\newcommand{\val}[1]{\mathit{v}\left({#1}\right)}
\newcommand{\vals}{\mathit{v}}
\newcommand{\zal}[1]{\mathit{z}\left({#1}\right)}
\newcommand{\zalt}[2]{\za_{#2}{\left(#1\right)}}
\newcommand{\zalts}[1]{\za_{#1}}
\newcommand{\zals}{\za}
\DeclareMathOperator{\za}{\mathit{z}}
\DeclareMathOperator{\vt}{\tilde{v}}


%%Dynamics

\DeclareMathOperator{\fct}{a}
\DeclareMathOperator{\Bct}{B}
\DeclareMathOperator{\Cct}{C}
\DeclareMathOperator{\Dct}{D}
\DeclareMathOperator{\Detf}{f}
\newcommand{\Pt}[2]{\Ptrans\left({#1}|{#2}\right)}
\newcommand{\Pts}[1]{\Ptrans\left({#1}\right)}
\DeclareMathOperator{\Ptrans}{\mathbb{P}}
\newcommand{\Detff}[4]{\dynf\left({#1},{#2},{#3},{#4}\right)}
\newcommand{\Pn}{\mathbb{P}_{\noisew}}
\newcommand{\PnS}{\tilde{\Sigma}}
\newcommand{\dynf}{\mathcal{F}}
\newcommand{\feats}{\phi}
\newcommand{\feat}[2]{\feats\left({#1},{#2}\right)}




%%  Decentralized   Control     Notation    %%

\DeclareMathOperator{\Kd}{\mathcal{K}}
\DeclareMathOperator{\K}{K}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Acal}[2]{F\left({#1}\right)}
\newcommand{\Bcal}[2]{G\left({#1}\right)}
\newcommand{\Aca}{F}
\newcommand{\Bca}{G}
\newcommand{\FP}[1]{\rho\left({#1}\right)}
\newcommand{\Ab}{\mathcal{S}}
\newcommand{\Htwo}{\mathcal{H}_2}
\newcommand{\Hinf}{\mathcal{H}_\infty}
\newcommand{\LQR}{\mathrm{LQR}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\Ad}{\tilde{A}}
\newcommand{\FHinf}[1]{q_\infty}
\newcommand{\FHtwo}[1]{q_2}
\newcommand{\FHone}[1]{q_1}
\newcommand{\FCtwo}[1]{q^c_2\left({#1}\right)}
\newcommand{\FCinf}[1]{q^c_\infty\left({#1}\right)}
\DeclareMathOperator{\Adts}{\tilde{\mathcal{A}}}
\DeclareMathOperator{\Ats}{\tilde{A}}
\DeclareMathOperator{\A}{A}
\DeclareMathOperator{\Bd}{\mathcal{B}}
\DeclareMathOperator{\B}{B}
\newcommand{\Sigmab}[1]{\Sigma_{\mathrm{big}}\left({#1}\right)}
\newcommand{\SigmaAltb}[1]{\tilde{\Sigma}_{\mathrm{big}}\left({#1}\right)}
\DeclareMathOperator{\Sigmain}{\Sigma_{in}}
\DeclareMathOperator{\Sigmaint}{\tilde{\Sigma_{in}}}
\DeclareMathOperator{\Sigmat}{\tilde{\Sigma}}
\newcommand{\Unoise}{\Sigma}
\newcommand{\Unoisei}{S}
\newcommand{\mup}{\overline{m}}
\newcommand{\md}{\underline{m}} 

==> TPWRS - Feasibility 2015/Notation.tex <==
%!TEX root=ConvexEnergyFunction.tex

\usepackage{accents}

\newcommand{\nf}{k}
%\newcommand{\VV}{VVPV}
%\newcommand{\IV}{Injection Vector}

\newcommand{\Poly}[2]{\mathrm{Poly}^{#2}\br{#1}}
\newcommand{\normnuc}[1]{\left\|{#1}\right\|_\text{nuc}}
\newcommand{\DSF}{DSF}
\newcommand{\SFe}{SF}
\newcommand{\Ly}[1]{\mathcal{L}_y\br{#1}}
\newcommand{\hermb}[1]{{#1}^{\mathcal{H}}}


\newcommand\munderbar[1]{%
  \underaccent{\bar}{#1}}
  
  \newcommand{\pqq}{\mathrm{pqq}}

\newcommand{\ygu}{y}
\newcommand{\opta}[1]{{#1}^{\ast}_{\risk}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\G}{\mathrm{pv}}
\newcommand{\NSB}{\mathrm{nsb}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\Vpf}{V^{\mathrm{pf}}}
\newcommand{\Vs}{\mathcal{V}}
\newcommand{\Submat}[3]{\left[{#1}\right]^{#2}_{#3}}

\newcommand{\Lo}{\mathrm{pq}}
\newcommand{\Vl}{\underline{V}}
\newcommand{\Vset}{v}
\newcommand{\Vdif}{\zeta}
\newcommand{\Vpow}{\beta}
\newcommand{\Bt}{\tilde{B}}
\newcommand{\Qt}{\tilde{Q}}
\newcommand{\af}{\alpha}
\newcommand{\df}{\delta}
\newcommand{\Aa}{A^1}
\newcommand{\Ac}{A^2}
\newcommand{\Int}{\mathrm{Int}}
\newcommand{\Sb}{\mathcal{S}}
\newcommand{\Mat}[3]{{\left[{#1}\right]}_{#2}^{#3}}
\newcommand{\Rep}[1]{\mathrm{Re}\br{#1}}
\newcommand{\Imp}[1]{\mathrm{Im}\br{#1}}
\newcommand{\Jac}[2]{\nabla {#1}\br{#2}}
\newcommand{\smi}{s}
\newcommand{\sma}{S}
\newcommand{\rl}{\underline{\rho}}
\newcommand{\ru}{\overline{\rho}}
\newcommand{\Vx}{V^x}
\newcommand{\Vy}{V^y}
\newcommand{\Vc}{V^c}
\newcommand{\Vml}{\rho}
\newcommand{\Vpl}{\theta}
\newcommand{\Ql}{\underline{q}}
\newcommand{\Qu}{\overline{q}}
\newcommand{\Pl}{\underline{p}}
\newcommand{\Pu}{\overline{p}}


\newcommand{\PQ}{PQ}
\newcommand{\PV}{PV}
\newcommand{\herm}[1]{{#1}^\ast}
\newcommand{\tim}{\otimes}

\newcommand{\Vref}{V_0}

\newcommand{\Com}{\mathbb{C}}


\newcommand{\Ind}[1]{\mathbb{I}\br{#1}}

\newcommand{\stc}[2]{\begin{pmatrix}
	{#1}\\{#2}
\end{pmatrix}}

\newcommand{\Conv}[1]{\text{Conv}\br{#1}}

\newcommand{\Cop}{\C_{op}}

\newcommand{\Pa}{W}
\newcommand{\Qa}{R}
\newcommand{\Ra}{Y}
\newcommand{\Ta}{T}
\newcommand{\Pat}{\tilde{W}}
\newcommand{\Vo}{v}
\newcommand{\Vco}{\Vc\br{0}}
\newcommand{\Vox}{v^x}
\newcommand{\Voy}{v^y}
\newcommand{\Vocs}{v^{nb}}
\newcommand{\Vocf}{v^{fb}}
\newcommand{\Vcs}{V^{nb}}
\newcommand{\Vcf}{V^{fb}}

\newcommand{\Mt}{\tilde{M}}
\newcommand{\Nt}{\tilde{N}}
\newcommand{\J}{J}
\newcommand{\JF}{J_F}
\newcommand{\JH}{J_H}
\newcommand{\JG}{J_{\Hc}}
\newcommand{\Hc}{H^{eq}}
\newcommand{\Fc}{H^{op}}


\newcommand{\ub}{\bar{V}}
\newcommand{\lb}{\munderbar{V}}
\newcommand{\fb}{\bar{f}}


\newcommand{\sub}{\kappa^u}
\newcommand{\slb}{\kappa^n}
\newcommand{\sfb}{\kappa^f}

\newcommand{\sP}{W}
\newcommand{\dio}[1]{\mathrm{di}^0\br{#1}}
\newcommand{\Gax}{G_{ax}}
\newcommand{\Gbx}{G_{bx}}
\newcommand{\Gby}{G_{by}}
\newcommand{\Gay}{G_{ay}}
\newcommand{\Bax}{B_{ax}}
\newcommand{\Bbx}{B_{bx}}
\newcommand{\Bby}{B_{by}}
\newcommand{\Bay}{B_{ay}}

\newcommand{\Aind}{A}
\newcommand{\aScal}{\mathcal{S}_a}

\newcommand{\Mu}{\Delta}

\newcommand{\sinj}{s}
\newcommand{\sliml}{\munderbar{s}}
\newcommand{\slimu}{\bar{s}}

\newcommand{\zin}{z\br{0}}
\newcommand{\kappin}{\kappa\br{0}}

\newcommand{\QF}[2]{\mathcal{Q}\br{{#1};{#2}}}

==> TPWRS - Feasibility 2015/Packages.tex <==
%\usepackage{mathtools}
\usepackage{verbatim}
\usepackage{algorithm}
\usepackage{bm}
%\usepackage{algorithmic}
\usepackage{algpseudocode}
\usepackage[all]{xy}
\usepackage{url}
\usepackage{amsmath,amsthm,amssymb}
\usepackage{graphicx}
\usepackage{subcaption}

%%  Theorem Styles  %%

\newtheorem{thm}{Theorem}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{Thm}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{MyLem}{Lemma}
\newtheorem{lemma}{lemma}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{Def}{definition}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\theoremstyle{remark}
\newtheorem{assumption}{Assumption} 
